Using Session Types for Reasoning About Boundedness in the Pi-Calculus

The classes of depth-bounded and name-bounded processes are fragments of the pi-calculus for which some of the decision problems that are undecidable for the full calculus become decidable. P is depth-bounded at level k if every reduction sequence for P contains successor processes with at most k active nested restrictions. P is name-bounded at level k if every reduction sequence for P contains successor processes with at most k active bound names. Membership of these classes of processes is undecidable. In this paper we use binary session types to decise two type systems that give a sound characterization of the properties: If a process is well-typed in our first system, it is depth-bounded. If a process is well-typed in our second, more restrictive type system, it will also be name-bounded.

==> eptcsdata.tex <==
\providecommand{\firstpage}{67}
\providecommand{\publicationstatus}{K. Peters and S. Tini (Eds.): Combined Workshop on Expressiveness in\\ Concurrency and Structural Operational Semantics (EXPRESS/SOS 2017).\\
EPTCS 255, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.255.5}{10.4204/EPTCS.255.5}}

